A Survey of Quantization Methods for Efficient Neural Network Inference

As soon as abstract mathematical computations were adapted to computation on digital computers, the problem of efficient representation, manipulation, and communication of the numerical values in those computations arose. Strongly related to the problem of numerical representation is the problem of quantization: in what manner should a set of continuous real-valued numbers be distributed over a fixed discrete set of numbers to minimize the number of bits required and also to maximize the accuracy of the attendant computations? This perennial problem of quantization is particularly relevant whenever memory and/or computational resources are severely restricted, and it has come to the forefront in recent years due to the remarkable performance of Neural Network models in computer vision, natural language processing, and related areas. Moving from floating-point representations to low-precision fixed integer values represented in four bits or less holds the potential to reduce the memory footprint and latency by a factor of 16x; and, in fact, reductions of 4x to 8x are often realized in practice in these applications. Thus, it is not surprising that quantization has emerged recently as an important and very active sub-area of research in the efficient implementation of computations associated with Neural Networks. In this article, we survey approaches to the problem of quantizing the numerical values in deep Neural Network computations, covering the advantages/disadvantages of current methods. With this survey and its organization, we hope to have presented a useful snapshot of the current research in quantization for Neural Networks and to have given an intelligent organization to ease the evaluation of future research in this area.

==> makefile <==
compilePdfOptions=
compPdftex=pdflatex ${compilePdfOptions}
compile= ${compPdftex}

TARGET=bin/main.pdf
FILES=main.tex


.SECONDEXPANSION:

####################  COMPILE PDF  ######################

all: ${TARGET}

bin/%.pdf : ${FILES} # .figs_ 
	mkdir -p bin
	${compile}  $*
	-bibtex $*
	-bibtex $*
	${compile} $*
	${compile} $*
	#${compile} $*
	mv $*.pdf $@
	#make clean
	#open ${TARGET}
	@echo Done ....!


##############  EXTERNALIZE TIKZ-FIGURES  ###############

# TIKZ_FIGS_DIR=tikz_figs
# FIGS=$(shell grep -h '[:space:]*\\inputtikz' ${TIKZ_FIGS_DIR}/figures.tex | sed '1D' | \
#   sed s'/[:space:]*\\inputtikz{\(.*\)}{/\1/' )
# FIGSPDF=$(FIGS:%=%.pdf)
# 
# .figs_ : $(FIGSPDF)
# 	date &> .figs_
# 
# ${TIKZ_FIGS_DIR}/%.pdf : $$(word 1, $$(subst -, ,$${TIKZ_FIGS_DIR}/%)).tex
# 	${compile} --jobname=${TIKZ_FIGS_DIR}/$* \
# 	  '\newcommand{\fakejobname}{${TIKZ_FIGS_DIR}/$*}\input{${TIKZ_FIGS_DIR}/figures.tex}'
# 
########################  CLEAN  ########################

cleanall: clean
	rm -r -f bin/*.pdf ${TIKZ_FIGS_DIR}/*.pdf .figs_
	cd      figs/matlab && ./clean.sh
	cd tikz_figs/matlab && ./clean.sh
	@echo Cleaned All ....! 

clean:
	rm -f *.aux *.dvi *.blg *.out *.log */*.log */*/*.log *~ */*~
	@echo Cleaned ....! 


